Unconscious lie detection as an example of a widespread fallacy in the Neurosciences

Neuroscientists frequently use a certain statistical reasoning to establish the existence of distinct neuronal processes in the brain. We show that this reasoning is flawed and that the large corresponding literature needs reconsideration. We illustrate the fallacy with a recent study that received an enormous press coverage because it concluded that humans detect deceit better if they use unconscious processes instead of conscious deliberations. The study was published under a new open-data policy that enabled us to reanalyze the data with more appropriate methods. We found that unconscious performance was close to chance - just as the conscious performance. This illustrates the flaws of this widely used statistical reasoning, the benefits of open-data practices, and the need for careful reconsideration of studies using the same rationale.

==> vf-commands.tex <==
%
%
%
%
\newcommand{\STF}   [3]{$F(#1) = #2$, $#3$}               %
\newcommand{\STFeps}[4]{$F(#1) = #2$, $\epsilon=#3$, $#4$}%
\newcommand{\STt}   [3]{$t(#1) = #2$, $#3$}               %
%
%
\newenvironment{manlof}
{\begin{list}
    {\textbf{Figure \arabic{enumi}:}}
    { \usecounter{enumi}
      \setlength{\labelwidth}{2.4cm}
      \setlength{\labelsep}{0.4cm}
      \setlength{\leftmargin}{2.6cm}}}
  {\end{list}}
%
%
\newenvironment{CHANGED}
{\marginpar{\textbf{CHAN\-GED} $\Longrightarrow$}}
{\marginpar{$\Longleftarrow$ \textbf{CHAN\-GED}}}
%
%
\newcommand{\standardFig}[4]{
    \centerline{\includegraphics[scale=#2]{#3}}
    \caption{#4}
    \label{#1}
  }

\newcommand{\inserthere}[1]{
  \vspace{3mm} %
  \begin{center}
    \fbox{Insert #1 about here}
  \end{center}
  \vspace{3mm} %
}

\newcommand{\todo}[1]{{\bf TODO: #1}}
\newcommand{\off}[1]{}
\newcommand{\degree}{\ensuremath{^\circ}} %

\newcommand{\changespacing}[1]{
  \renewcommand{\baselinestretch}{#1} %
  \small\normalsize
}
\newcommand{\singlespaced}{\changespacing{1}}
\newcommand{\doublespaced}{\changespacing{2}}

%
\newcommand{\niceletter}[1]{
\begin{wrapfigure}[5]{l}{1.0cm}
{\fontencoding{U}\fontfamily{yinit}\fontseries{m}\fontshape{n}\selectfont #1}
\end{wrapfigure}}

\newcommand{\pressLink}[1]{ {\tiny \url{#1}}}
%

%
%
\makeatletter
\newcommand*{\citeNoSuperscript}[2][]{%
  \begingroup
  \let\NAT@mbox=\mbox
  \let\@cite\NAT@citenum
  \let\NAT@space\NAT@spacechar
  \let\NAT@super@kern\relax
  \renewcommand\NAT@open{}%
  \renewcommand\NAT@close{}%
  \cite[#1]{#2}%
  \endgroup
}
\makeatother


==> vf-header.tex <==
%
%
\newif\iflatextortf  %
\latextortffalse     %
%

%
%
%
%
%
\usepackage[latin1]{inputenc}  %
%
%
%
%
%
%
%
\sloppy

%
%
\usepackage[american]{babel} %

%
\raggedright
\setlength{\parindent}{2em}
%
%

%
%
%
%
%
%
%
%
%
%
%
%
\usepackage[sort&compress]{natbib}
\bibliographystyle{unsrtnat}
\bibpunct{(}{)}{,}{n}{}{}
%
%
%
%

%
\renewcommand*{\thefootnote}{\fnsymbol{footnote}}

%
\iflatextortf
  %
\else
  \usepackage{setspace}
  %
  %
  %
\fi

\usepackage[T1]{fontenc} 

%
\usepackage[pdftex]{graphicx}
%
%

%
\draftsubmit{
  %
  \newcommand{\figureLabels}[2]{\vfill{}{\large Figure: #1; File: #2}}
  \newcommand{\draftComment}[1]{#1}
}{
  %
  \newcommand{\figureLabels}[2]{\vfill{}{\small Figure: #1}}
  \newcommand{\draftComment}[1]{}
}

%
%
\draftsubmit{
  %
%
  \def\boxit{}
}{
  %
  \def\boxit{}
}

%
%
\draftsubmit{
  %
  \def\scaleit{1}
  %
}{
  %
  \def\scaleit{1}
}

%
\coverlettermarksoffon{
  %
  \newcommand{\coverlettermark}[1]{}
}{
  %
  \newtheorem{cvtheor}{$\bullet$ mark} %
  \newcommand{\coverlettermark}[1]{
    \marginpar{
      \parbox{1.8cm}{
        \renewcommand{\baselinestretch}{1} %
        \begin{cvtheor}
          \label{#1}
        \end{cvtheor}}}}
}

%
\draftsubmit{
  %
  \def\SubmissionBanner{\vfill 
    \begin{center}
      \textbf{\large 
        Draft \\
        Please do not cite or distribute!
      }\end{center}}
}{
  %
  \def\SubmissionBanner{}
}
%
\hyphenation{elec-tro-en-ce-pha-lo-gra-phy}

